Hardware-Oriented Krylov Methods for High-Performance Computing

Krylov subspace methods are an essential building block in numerical simulation software. The efficient utilization of modern hardware is a challenging problem in the development of these methods. In this work, we develop Krylov subspace methods to solve linear systems with multiple right-hand sides, tailored to modern hardware in high-performance computing. To this end, we analyze an innovative block Krylov subspace framework that allows to balance the computational and data-transfer costs to the hardware. Based on the framework, we formulate commonly used Krylov methods. For the CG and BiCGStab methods, we introduce a novel stabilization approach as an alternative to a deflation strategy. This helps us to retain the block size, thus leading to a simpler and more efficient implementation. In addition, we optimize the methods further for distributed memory systems and the communication overhead. For the CG method, we analyze approaches to overlap the communication and computation and present multiple variants of the CG method, which differ in their communication properties. Furthermore, we present optimizations of the orthogonalization procedure in the GMRes method. Beside introducing a pipelined Gram-Schmidt variant that overlaps the global communication with the computation of inner products, we present a novel orthonormalization method based on the TSQR algorithm, which is communication-optimal and stable. For all optimized method, we present tests that show their superiority in a distributed setting.

==> generated/gmres_hybrid_vs_global/gmres_hybrid_vs_global.tex <==
\begin{tabular}{lcc|cc}
\toprule
{} & \multicolumn{2}{l}{block-global} & \multicolumn{2}{l}{block-parallel} \\
{} &          $t$ & iterations &            $t$ & iterations \\
$p$ &              &            &                &            \\
\midrule
1   &      48.6994 &         60 &        31.7917 &         47 \\
2   &     917.6630 &         60 &       464.8530 &         42 \\
4   &    1062.8600 &         59 &       381.3530 &         35 \\
8   &      54.0240 &         56 &        17.6836 &         26 \\
16  &      39.5586 &         42 &        13.0052 &         18 \\
32  &      33.7360 &         35 &        10.8330 &         14 \\
64  &      17.5402 &         18 &        10.2902 &         11 \\
128 &      12.3335 &         11 &        10.8852 &          9 \\
256 &      14.6942 &          8 &        14.4182 &          8 \\
\bottomrule
\end{tabular}


==> texFiles/dedication.tex <==
%!TEX root = ../thesis.tex
\makededication{for someone!}

==> texFiles/globaltodo.tex <==
\todo[inline]{consistency complex numbers (check transpose and conjugate)}
\todo[inline]{check all algorithms!}


%%% Local Variables:
%%% mode: latex
%%% TeX-command-extra-options: "-usepretex='\\includeonly{texFiles/globaltodo.tex}'"
%%% TeX-master: "../thesis"
%%% End:

==> texFiles/keywords.tex <==
%!TEX root = ../thesis.tex
\makekeywords{some keywords} 


==> texFiles/statementOfAuthorship.tex <==
%!TEX root = ../thesis.tex
\chapter*{Eidesstattliche Erklärung}

Hiermit versichere ich, \textit{\mthauthor}, dass ich die vorliegende Arbeit selbst\-ständig verfasst und keine anderen als die angegebenen Quellen und Hilfsmittel verwendet habe. Gedanklich, inhaltlich oder wörtlich Übernommenes habe ich durch Angabe von Herkunft und Text oder Anmerkung belegt bzw. kenntlich gemacht. Dies gilt in gleicher Weise für Bilder, Tabellen, Zeichnungen und Skizzen, die nicht von mir selbst erstellt wurden.\\
\ \\
Alle auf der CD beigefügten Programme sind von mir selbst programmiert oder durch Angabe von Herkunft kenntlich gemacht worden.

\par
\vspace*{10ex}

\begin{minipage}[b][][t]{0.45\textwidth}
	Münster, \mthdate
\end{minipage}
\hfill
\begin{minipage}[b][][b]{0.45\textwidth}
	\hrulefill
\end{minipage}

\par
\vspace*{-1ex}
\hfill
\begin{minipage}{0.45\textwidth}
	\centering
	\mthauthor
\end{minipage}

==> texFiles/style/thesisColors.tex <==
%% define colors

% define WWU colors
\definecolor{wwuPantone7}{RGB}{62,62,59}
\definecolor{wwuPantone312}{RGB}{0,157,209}
\definecolor{wwuPantone315}{RGB}{0,110,137}
\definecolor{wwuPantone3135}{RGB}{0,142,150}
\definecolor{wwuPantone369}{RGB}{122,181,22}
\definecolor{wwuPantone390}{RGB}{177,200,0}
\definecolor{wwuPantone396}{RGB}{223,219,0}
\definecolor{wwuPantoneYellow}{RGB}{255,237,0}

\definecolor{wwuPantone234}{RGB}{175,0,120}
\definecolor{wwuPantone7462}{RGB}{0,87,138}


% define Solarized colorsceme
\definecolor{solBase03}{RGB}{0  43  54}
\definecolor{solBase02}{RGB}{7  54  66}
\definecolor{solBase01}{RGB}{88 110 117}
\definecolor{solBase00}{RGB}{101 123 131}
\definecolor{solBase0}{RGB}{131 148 150}
\definecolor{solBase1}{RGB}{147 161 161}
\definecolor{solBase2}{RGB}{238 232 213}
\definecolor{solBase3}{RGB}{253 246 227}
\definecolor{solYellow}{RGB}{181 137   0}
\definecolor{solOrange}{RGB}{203  75  22}
\definecolor{solRed}{RGB}{220  50  47}
\definecolor{solMagenta}{RGB}{211  54 130}
\definecolor{solViolet}{RGB}{108 113 196}
\definecolor{solBlue}{RGB}{38 139 210}
\definecolor{solCyan}{RGB}{42 161 152}
\definecolor{solGreen}{RGB}{133 153   0}


% define own colors
\definecolor{set1color1}{RGB}{237, 106, 90}
\definecolor{set1color2}{RGB}{12, 124, 89}
\definecolor{set1color3}{RGB}{112, 171, 175}
\definecolor{set1color4}{RGB}{87, 90, 75}
\definecolor{set1color5}{RGB}{186, 193, 184}


% define colors used for document
\definecolor{highlightColorRed}{named}{set1color1}
\definecolor{highlightColorGreen}{named}{set1color2}
\definecolor{highlightColorBlue}{named}{set1color3}
\definecolor{highlightColor}{named}{highlightColorRed}
\definecolor{mainColor}{named}{wwuPantone7}
\definecolor{backgroundColor}{named}{set1color5}

% define colors for listings
\definecolor{cppcommentcolor}{RGB}{00 64 00}

% define colors for tiks figures
\newcommand\tikzColorSat{1}
\newcommand\tikzColorBrightness{1}
\definecolor{tikzcolor1}{hsb}{0.0,\tikzColorSat,\tikzColorBrightness}
\definecolor{tikzcolor2}{hsb}{0.0625,\tikzColorSat,\tikzColorBrightness}
\definecolor{tikzcolor3}{hsb}{0.125,\tikzColorSat,\tikzColorBrightness}
\definecolor{tikzcolor4}{hsb}{0.1875,\tikzColorSat,\tikzColorBrightness}
\definecolor{tikzcolor5}{hsb}{0.25,\tikzColorSat,\tikzColorBrightness}
\definecolor{tikzcolor6}{hsb}{0.3125,\tikzColorSat,\tikzColorBrightness}
\definecolor{tikzcolor7}{hsb}{0.375,\tikzColorSat,\tikzColorBrightness}
\definecolor{tikzcolor8}{hsb}{0.4375,\tikzColorSat,\tikzColorBrightness}
\definecolor{tikzcolor9}{hsb}{0.5,\tikzColorSat,\tikzColorBrightness}
\definecolor{tikzcolor10}{hsb}{0.5625,\tikzColorSat,\tikzColorBrightness}
\definecolor{tikzcolor11}{hsb}{0.625,\tikzColorSat,\tikzColorBrightness}
\definecolor{tikzcolor12}{hsb}{0.6875,\tikzColorSat,\tikzColorBrightness}
\definecolor{tikzcolor13}{hsb}{0.75,\tikzColorSat,\tikzColorBrightness}
\definecolor{tikzcolor14}{hsb}{0.8125,\tikzColorSat,\tikzColorBrightness}
\definecolor{tikzcolor15}{hsb}{0.875,\tikzColorSat,\tikzColorBrightness}
\definecolor{tikzcolor16}{hsb}{0.9375,\tikzColorSat,\tikzColorBrightness}

